CURE-OR: Challenging Unreal and Real Environments for Object Recognition

In this paper, we introduce a large-scale, controlled, and multi-platform object recognition dataset denoted as Challenging Unreal and Real Environments for Object Recognition (CURE-OR). In this dataset, there are 1,000,000 images of 100 objects with varying size, color, and texture that are positioned in five different orientations and captured using five devices including a webcam, a DSLR, and three smartphone cameras in real-world (real) and studio (unreal) environments. The controlled challenging conditions include underexposure, overexposure, blur, contrast, dirty lens, image noise, resizing, and loss of color information. We utilize CURE-OR dataset to test recognition APIs-Amazon Rekognition and Microsoft Azure Computer Vision- and show that their performance significantly degrades under challenging conditions. Moreover, we investigate the relationship between object recognition and image quality and show that objective quality algorithms can estimate recognition performance under certain photometric challenging conditions. The dataset is publicly available at https://ghassanalregib.com/cure-or/.

==> Preprint for arXiv/cure_or.tex <==
%\subsection{Objects}\label{subsec:objects}
\noindent{\bf Objects:}~\texttt{CURE-OR} dataset includes 100 objects of different color, size, and texture as shown in Fig. \ref{fig:objects}. The objects are grouped into 6 categories as toys, personal belongings, office supplies, household items, sports/entertainment items, and health/personal care items. The number of objects in each category varies between $10$ and $24$. For more details,  please refer to  \href{https://ghassanalregib.com/cure-or/}{https://ghassanalregib.com/cure-or/}. 




%\subsection{Acquisition Devices and Data Format}
% Device names, the setup with devices (slightly varying angles), data format/resolution (original resolution & downsampled resolution)
%\vspace{3mm}
\vspace{1mm}
\noindent{\bf Acquisition setup and image format:}~The images in \texttt{CURE-OR} were captured with 5 devices including iPhone 6s, HTC One X, LG Leon, Logitech C920 HD Pro Webcam, and Nikon D80, which were mounted on a Vanguard multi-mount horizontal bar attached to a tripod and controlled with wireless remotes. Each device had a slightly different perspective because of their relative locations. Images were captured in real and unreal environments. First, images were captured in a photo studio setup (LITEBOX Pro-240) with a white backdrop and two realistic backdrops of living room and kitchen. Second, images were captured in real-world environments including a living room and an office setup. The sample images of an object in every background are shown in Fig. \ref{fig:backgrounds}. Objects were captured at 5 different orientations: front, back, top, left-side, and right-side views. Originally, the width and height of captured images vary from $1,840$ to $5,168$ pixels with an average resolution of $2,457 \times 3,785 $. These images were scaled down to 1/4 of their original resolution and stored as JPEG to reduce dataset size.  

\vspace{-1mm}
\begin{figure}[htbp!]
%\begin{adjustbox}{minipage=\linewidth-4pt,margin=5pt 5pt,bgcolor=blue_2,frame=0pt}
    \begin{minipage}[t]{0.18\linewidth}
      \centering
    \includegraphics[width=\textwidth]{./Figs/Backgrounds/1_1_2_007.jpg}
      \vspace{0.01cm}
      \centerline{\footnotesize{(a)
    {\tabular[t]{@{}l@{}} White\\  \endtabular}}}%\medskip
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.18\linewidth}
      \centering
    \includegraphics[width=\textwidth]{./Figs/Backgrounds/2_1_2_007.jpg}
      \vspace{0.01cm}
      \centerline{\footnotesize{(b)
      {\tabular[t]{@{}l@{}} Living\\ Room  \endtabular}}}%\medskip
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.18\linewidth}
      \centering
    \includegraphics[width=\linewidth]{./Figs/Backgrounds/3_1_2_007.jpg}
      \vspace{0.01 cm}
      \centerline{\footnotesize{(c)
      {\tabular[t]{@{}l@{}} Kitchen\\ \endtabular}}}%\medskip
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.18\linewidth}
      \centering
    \includegraphics[width=\linewidth]{./Figs/Backgrounds/4_1_2_007.jpg}
      \vspace{0.01 cm}
      \centerline{\footnotesize{(d)
      {\tabular[t]{@{}l@{}} Living \\ Room  \endtabular}}}%\medskip
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.18\linewidth}
      \centering
    \includegraphics[width=\linewidth]{./Figs/Backgrounds/5_1_2_007.jpg}
      \vspace{0.01 cm}
      \centerline{\footnotesize{(e)
      {\tabular[t]{@{}l@{}} Office \\    \endtabular}}}%\medskip
    \end{minipage}
    \centering
      \vspace{-1.0mm}
    \caption{ Studio (a)-(c) and real-world (d)-(e) environments.}
    \label{fig:backgrounds}
%\end{adjustbox}
\end{figure}
\vspace{-4mm}


% The 2D backgrounds refer to the setups with LITEBOX Pro-240 Light Box photo studio, which provides consistent lighting and allows to utilize different backdrops. While the photo studio set included PVC backdrops of various colors, only the white PVC backdrop was used as a plain background, and two more backdrops of living room and kitchen images were printed on poster paper to serve as textured backgrounds. Each printed backdrop has a table on the bottom whose edge was placed along the line in the back of the photo box for more realistic background. For the 3D backgrounds, two different spaces were created to simulate real-life scenarios of of using an object recognition application. A living room was created with a couch, a table with magazines where the objects of interest were placed, and another small table with a cup of coffee. An office setup was created with a desk placed in front of a bookshelf filled with books and assorted office supplies. 
 



%In each background, an object is captured at 5 different orientations: 4 side views at every 90 degrees rotating clockwise (0 degrees-front; 90 degrees-left; 180 degrees-back; and 270 degrees-right) and a top view. The side of an object with the most characteristic features was placed facing the cameras for the front view and was rotated 90 degrees clockwise for each of the other three side-view images. For the top view, an object was placed the same way as in the front view but was captured at a higher angle with the horizontal arm on the tripod rotated such that the cameras hang from the bar, facing toward floor.





%To minimize the variation in the setup between devices, including the background and object location and orientation, all devices were mounted on Vanguard multi-mount horizontal bar attached to a tripod and operated almost simultaneously with wireless remotes for image capture. Due to spatial limitation on the horizontal bar, however, each device has a slightly different angle toward objects in the setup. All devices except for Nikon D80 generate images of JPEG format, while Nikon D80 data format was chosen to be NEF format (Nikon Electronic Format; Nikon's RAW file format) in order to preserve as much as information possible and prevent the camera from applying in-camera processing. The NEF images from Nikon D80 were later converted into JPEG files to be consistent with other images in the dataset. The pixel dimensions of images from all devices range from 1,960 pixels to 5,168 pixels with most on the higher end, so each dimension of all images was scaled down to be a 1/4 of its original dimension for to keep the size of the dataset reasonable. 

%\subsection{Background Types and Object Orientations}
% Types of backgrounds, details on the setup (2d backdrops in the LiteBox, 3d space setups)

\input{fig_api_example_h.tex}

\vspace{1mm}
\noindent{\bf Challenges types:}
 Images in the \texttt{CURE-OR} dataset were separated into color and grayscale images to investigate the importance of color information in object recognition. We processed original images to simulate realistic challenging conditions including \emph{underexposure}, \emph{overexposure}, \emph{blur}, \emph{contrast}, \emph{dirty lens}, \emph{salt and pepper noise}, and \emph{resizing}. Brightness of images was adjusted to obtain \emph{underexposure} and \emph{overexposure} images. Pixel values were remapped to obtain \emph{contrast} images and smoothed out with a Gaussian operator to obtain \emph{blur} images. \emph{Dirty lens} images were obtained by overlaying dirty lens patterns over original images. In the first \emph{dirty lens} category, a single dirt pattern was blended into images with weights that were proportional to challenge levels. In the second category, a distinct dirt pattern was overlaid for each challenge level. In the \emph{salt and pepper} category, pixels were randomly replaced with zeros and ones. \emph{Salt and pepper noise} was synthesized with scikit-image version 0.13.0 and all other challenging conditions were simulated with Python Imaging Library version 4.2.1. 



%but original image category can also be considered as another level since it is already scaled down
\vspace{1mm}
\noindent{\bf Challenges levels:} The number of distinct challenge levels is 4 in \emph{resizing} category and 5 in all other categories. Challenge levels were adjusted based on visual inspection instead of numerical progression. Challenge level adjustment experiments were conducted by a group of three individuals, two experts and one intermediate in image processing, in an office space under standard lighting conditions. In the first experiment, we utilized a 65-inch LED TV display, whose settings were fixed to standard viewing conditions. We tuned the parameters in challenge generation such that challenges in level 1 were visible but they did not affect recognition, whereas in challenge level 5, objects were hardly recognizable or further changes in parameters did not correspond to significant perceivable difference. Mid challenge levels were linearly interpolated between min and max challenge levels. In the second experiment, we displayed level-1 and level-5 sample images on a 27-inch LCD PC monitor and observed that initial selection criteria still held in a different setup. In both experiments, subjects were located at a distance of twice the display size. Sample images corresponding to different challenge types and levels are shown in Fig. \ref{fig:challenges_api_h} with the API results that will be discussed in the following section. 


 %Only the color images are shown since the same challenge types and levels are applied to both color and grayscale sets of images.Resizing challenge is omitted since the sample images are not of original dimensions and would not deliver the significance of challenge in even more scaled down sample images. The level 4 and 5 are excluded since the following section utilizes images of challenge level 1 through 3 for the performance analysis of a recognition application.

 













%CURE-OR dataset is created by simulating different types of challenges using the original images in color and grayscale. The original images in color are used to generate grayscale images, still free of 8 types of challenges and used as references for the grayscale images with simulated challenges, although the removal of color is another type of challenge by itself. The original images in color and those in grayscale are grouped separately for further explanation of challenges as the same types and levels of challenges are applied to both. 

%For each group of the original images, 8 types of challenges are simulated---resizing, underexposure, overexposure, blur, contrast, two different dirty lens effects, and salt and pepper noise. 

%All challenging conditions except salt and pepper noise are generated using Python Imaging Library version 4.2.1, and salt and pepper noise challenge is simulated with scikit-image version 0.13.0. \textbf{Reference: PIL \& scikit-image} 


%Resizing challenge reduces the pixel dimensions of an image by factors of values between 1 (exclusive) and 0.5 (inclusive). 

%Both exposure challenges control the brightness in an image, brighter for overexposure and darker for underexposure.Blur challenge implements Gaussian blur with different radius sizes. Contrast challenge adjusts the contrast of an image by further separating dark colors and bright colors on spectrum. The first dirty lens challenge blends an image of dirty lens effect onto an original image with increasing weight factors for more severe challenge levels. The second dirty lens challenge overlays a combination of 5 distinct transparent dirty lens effect, with one effect image being the lowest challenge level and all five effect images the most significant.Salt and pepper challenge replaces random pixels of an image with either 1 or 0.



%  \input{fig_challenges_h.tex}


%\input{fig_challenges_h.tex}

% \textbf{8 challenges: challenge generation process/type; challenge level selection process}

% Figure \ref{fig:challenges} \textbf{Figure: resizing not shown, as well as example images in grayscale}






==> Preprint for arXiv/fig_api_example_h.tex <==
% https://tex.stackexchange.com/questions/239715/add-titles-for-rows-and-columns-in-a-subfloat
\newlength{\imgHeight}
\newlength{\imgWidth}
\newlength{\resWidth}
\newlength{\vblank}
\newlength{\cTypeHeight}
\newlength{\levelWidth}

\newcommand{\columnname}[1]% #1 = text
{\begin{minipage}[c][\cTypeHeight][t]{\imgWidth+\resWidth}\makebox[\imgWidth][c]{\textbf{\small#1}}\end{minipage}}

\newcommand{\rowname}[1]% #1 = text
{\begin{minipage}[b]{\levelWidth}
    \centering\rotatebox{90}{\makebox[\imgHeight][c]{\textbf{\small#1}}}
\end{minipage}}

\newcommand{\populateRow}[1]
{
    {\includegraphics[trim=0 0 0 3cm,clip,width=\imgWidth]{./Figs/api_example/2_5_2_069_03_#1.jpg}}\vspace{\vblank}\hfill
    {\includegraphics[trim=5mm 5mm 5mm 5mm,clip,height=\imgHeight]{./Figs/api_example_bar/03_#1.pdf}}\hfill
    {\includegraphics[trim=0 0 0 3cm,clip,width=\imgWidth]{./Figs/api_example/2_5_2_069_04_#1.jpg}}\hfill
    {\includegraphics[trim=5mm 5mm 5mm 5mm,clip,height=\imgHeight]{./Figs/api_example_bar/04_#1.pdf}}\hfill
    {\includegraphics[trim=0 0 0 9mm,clip,width=\imgWidth]{./Figs/api_example/2_5_2_069_05_#1.jpg}}\hfill
    {\includegraphics[trim=5mm 5mm 5mm 5mm,clip,height=\imgHeight]{./Figs/api_example_bar/05_#1.pdf}}\hfill
    {\includegraphics[trim=0 0 0 3cm,clip,width=\imgWidth]{./Figs/api_example/2_5_2_069_06_#1.jpg}}\hfill
    {\includegraphics[trim=5mm 5mm 5mm 5mm,clip,height=\imgHeight]{./Figs/api_example_bar/06_#1.pdf}}\hfill
    {\includegraphics[trim=0 0 0 9mm,clip,width=\imgWidth]{./Figs/api_example/2_5_2_069_07_#1.jpg}}\hfill
    {\includegraphics[trim=5mm 5mm 5mm 5mm,clip,height=\imgHeight]{./Figs/api_example_bar/07_#1.pdf}}\hfill
    {\includegraphics[trim=0 0 0 9mm,clip,width=\imgWidth]{./Figs/api_example/2_5_2_069_08_#1.jpg}}\hfill
    {\includegraphics[trim=5mm 5mm 5mm 5mm,clip,height=\imgHeight]{./Figs/api_example_bar/08_#1.pdf}}\hfill
    {\includegraphics[trim=0 0 0 3cm,clip,width=\imgWidth]{./Figs/api_example/2_5_2_069_09_#1.jpg}}\hfill
    {\includegraphics[trim=5mm 5mm 5mm 5mm,clip,height=\imgHeight]{./Figs/api_example_bar/09_#1.pdf}}\\
}


\begin{figure*}[!htbp]
% \begin{adjustbox}{minipage=\linewidth-8pt,margin=2pt 2pt,bgcolor=blue_2,frame=0pt}

    \setlength{\imgWidth}{.1\linewidth}
    \settoheight{\imgHeight}{\includegraphics[trim=0 0 0 3cm,clip,width=\imgWidth]
        {./Figs/api_example/2_5_2_069_03_1.jpg}}
    \setlength{\resWidth}{.02\linewidth}
    \setlength{\vblank}{0.5mm}
    \setlength{\cTypeHeight}{4mm}
    \setlength{\levelWidth}{5mm}

    \begin{minipage}[b]{\levelWidth}\centering{\makebox[5mm][c]{}}\end{minipage}
        \columnname{Underexposure}\hfill
        \columnname{Overexposure}\hfill
        \columnname{Blur}\hfill
        \columnname{Contrast}\hfill
        \columnname{Dirty Lens 1}\hfill
        \columnname{Dirty Lens 2}\hfill
        \columnname{Salt \& Pepper}\\
    \rowname{Level 1}\populateRow{1}
    \rowname{Level 2}\populateRow{2}
    \rowname{Level 3}\populateRow{3}
    \rowname{Level 4}\populateRow{4}
    \rowname{Level 5}\populateRow{5}
\vspace{-4mm}
\caption{Sample images with challenging conditions (levels 1-5). The labels on the right side of each image are the top-1 output from Amazon Rekognition and Microsoft Azure Computer Vision. The labels in blue are considered correct for the selected object and those in yellow are considered incorrect.}
\label{fig:challenges_api_h}
% \end{adjustbox}
\vspace{-4mm}
\end{figure*} 

==> Preprint for arXiv/intro.tex <==
Recent advancements in algorithms and hardware platforms led to the development of state-of-the-art visual recognition methods that can achieve human-level performance in specific recognition tasks \cite{He2015,Wu2015}. Traditionally, these state-of-the-art recognition approaches were based on handcrafted features such as SIFT \cite{Lowe2004}, SURF \cite{Bay2006} and HoG \cite{Dalal2005}. However, recent data-driven methods started to outperform handcrafted methods as in the ImageNet Large Scale Visual Recognition Challenge (ILSVRC) \cite{Deng2009}. There are numerous datasets similar to ImageNet \cite{Li2004,Opelt2005,Everingham2005,Russell2008,Torralba2008,Krizhevsky09,Deng2009,Saenko2010,Lin2014}, whose images were obtained through photo sharing platforms and search engines. Even though these datasets can be comprehensive in terms of number of samples per categories, it is not possible to identify the relationship between specific conditions and recognition performance because of their uncontrolled nature. However, challenging conditions can significantly degrade the recognition performance as discussed in Section \ref{sec:exp}. Therefore, to investigate the robustness of recognition algorithms with respect to challenging conditions, we need to perform controlled experiments that include a comprehensive set of challenging condition types and levels.
% \vspace{-1mm}


%Majority of these datasets are limited in terms of challenging conditions. There is usually no metadata corresponding to challenge conditions or levels in these datasets. Moreover, the relationship between challenging conditions and algorithmic performance is not analyzed in these studies. 



%Specifically, the popularity of deep learning approaches significantly increased after their top performances in visual object recognition competitions \cite{Deng2009,Everingham2005}. 

\begin{comment}
\begin{figure}[htbp!]
     \vspace{-1.0mm}
    \centering
    \includegraphics[width=0.65\linewidth, trim= 0mm 0mm 0mm 10mm]{./Figs/Overall_performance.pdf}\vspace{-4 mm}
    \caption{Top 5 recognition accuracy of Amazon Rekognition under challenging conditions in the CURE-OR dataset.}
    \label{fig:cure_bar}
    \vspace{-3.0mm}
\end{figure}
\end{comment}

 

Recent studies started investigating the effect of challenging conditions in images in terms of recognition performance \cite{Hosseini2017,Dodge2016,Zhou2017,Lu2017,Das2017,Temel2017_NIPSW}.  Hosseini \textit{et al.} \cite{Hosseini2017} evaluated the recognition performance of Google Cloud Vision API under Gaussian and impulse noise and showed that the API is vulnerable to tested challenging conditions. Dodge and Karam \cite{Dodge2016} evaluated the recognition performance of deep neural networks under blur, noise, contrast, and compression and showed that deep learning-based approaches are susceptible to degradation, particularly to blur and noise. Zhou \textit{et al.} \cite{Zhou2017} also studied the effect of blur and noise in deep network-based recognition and showed their vulnerabilities. Similarly, Lu \textit{et al.} \cite{Lu2017} and Das \textit{et al.} \cite{Das2017} showed the vulnerability of traffic sign recognition and detection systems in case of adversarial examples. Even though these studies shed light on a subset of conditions that can significantly affect algorithmic performance, the investigated challenging conditions are relatively limited. Specifically, aforementioned studies \cite{Hosseini2017,Dodge2016,Zhou2017,Lu2017,Das2017} focus on simulated challenging conditions and they overlook the possible imperfections in the acquisition process. Moreover, adversarial examples investigated in \cite{Lu2017,Das2017} are inherently different from realistic challenging scenarios because they are specifically tuned to bias the models. Temel \textit{et al.} \cite{Temel2017_NIPSW} focus on realistic challenging conditions but the application field is limited to traffic signs. Therefore, we need more comprehensive robustness analysis for generic object recognition tasks that considers realistic conditions as well as nonidealities in the acquisition processes.




\vspace{1mm}
This paper has three major components: the newly built \texttt{CURE-OR} dataset by which we eliminate the shortcomings of existing datasets; the performance benchmark of object recognition on the new dataset using the recognition APIs Amazon Rekognition and Microsoft Azure Computer Vision; and the investigation of the relationship between object recognition performance and full-reference image quality assessment, which measure the changes with respect to a challenge-free reference image. If we consider ideal conditions as reference conditions and non-ideal conditions as photometric challenging conditions, image quality should decrease under challenging conditions. \emph{Based on this assumption related to image quality, we hypothesize that object recognition performance under photometric challenging conditions can be estimated with objective image quality assessment algorithms.} Specifically, we focus on photometric challenging conditions including \emph{blurriness}, \emph{dirtiness of lens}, \emph{contrast}, \emph{overexposure}, \emph{undersexposure}, and \emph{sensor noise}. The contributions of this paper are five folds.

\vspace{2 mm}

\begin{itemize}[label=\textcolor{orange}{\FilledSmallSquare},leftmargin=*]   \setlength\itemsep{0.45em}
\item We introduce the most \emph{comprehensive} publicly-available object recognition dataset acquired with multiple device types under controlled challenging conditions in \emph{real-world} and \emph{photo studio} environments.

\item We provide a detailed description and a \emph{comparative} study of existing object datasets,  which  can  be  used as a source of reference in further studies.   

\item We provide a detailed \emph{analysis} of \emph{recognition APIs} in terms of recognition performance under challenging conditions. 
   

\item We show that the performance of recognition applications significantly \emph{degrades} under challenging conditions.
    
\item We utilize full-reference objective \emph{image quality} assessment algorithms to \emph{estimate} the object recognition \emph{performance} under \emph{photometric} challenging conditions.
\end{itemize}

\vspace{2 mm}
 
\noindent{\bf Outline:}~We briefly discuss existing object datasets in Section~\ref{sec:related_work}. In Section~ \ref{sec:cure-or}, we introduce and describe the \texttt{CURE-OR} dataset. We analyze the performance of recognition APIs under challenging conditions in Section~\ref{sec:exp}, and we investigate the relationship between object recognition performance and objective quality assessment in Section~\ref{sec:quality}. Finally, we conclude our work in Section~\ref{sec:conc}.    





 


==> Preprint for arXiv/main_1.tex <==
There are numerous visual recognition applications that are publicly available, but it is not feasible to perform large-scale experiments in majority of these applications. After a preliminary feasibility study, we conducted our experiments using
\href{https://aws.amazon.com/rekognition/}{Amazon Rekognition API (AMZN)} and \href{https://azure.microsoft.com/en-us/services/cognitive-services/computer-vision/}{Microsoft Azure Computer Vision API (MSFT)}. Rekognition is a deep learning-based image recognition system provided by Amazon Web Services. Microsoft Azure Computer Vision utilizes image processing algorithms to analyze visual contents. We use the object recognition feature from AMZN and the image tagging functionality from MSFT to assess their performance.

\subsection{Experimental Setup}
\label{subsec:challenge_setup}
% 24 objects - 8 challenges each in color and grayscale

%% Amazon Rekognition experiment process (ground truth label collection, etc.)


\noindent{\bf Test Set:} For both APIs, we input challenge-free images of 100 objects from CURE-OR dataset to collect object labels, and analyzed the collected labels semantically to identify the labels that can be considered ground truth. For example, a Coca Cola bottle can be recognized as a beverage, a bottle, a drink, a coke, a soda, or a glass. We selected 4 objects from each object category based on the number of images that can be correctly identified by each API. If a selected object was similar to another object in the same category, the object with more correctly identified images was utilized. Microsoft identified only 3 objects in health/personal care category, so one object with the least number of correctly identified images from Amazon was excluded for a fair analysis, which led to 23 objects (top objects) selected for each API. For direct comparison of the platforms, we also analyzed the recognition performance on the 10 common objects between the 23 top objects of both APIs. In total, we tested the performance of each API with $230,000$ images. 
% There were 6,000 ($24~objects~\times~5~backgrounds~\times~5~devices~\times~5~orientations$ $~\times~2~color/grayscale$  ) challenge-free images and 144,000 ($24~objects~\times~5~backgrounds~\times~5~devices~\times~5~orientations$ $~\times~2~color/grayscale~\times~8~ challenge~types~\times~3~challenge$ $~levels$) images with controlled challenging conditions. 
We limited the number of tested objects to minimize the total cost of the experiment using Amazon. However, we were able to test the recognition performance for the remaining images using Microsoft thanks to promotional credits. On average, testing per image took 1.3 seconds for Amazon and 0.2 seconds for Microsoft. 



\begin{comment}
AWS: 82.8 hours for 230,000 images
Azure: 13.8 hours for 230,000 images
       60 hours for 1,000,000 images
\end{comment}


% ~Amazon Rekognition API has \emph{DetectLabels} operation that analyzes an image to detect objects and generates an output of collected object labels with respective confidence levels. We input challenge-free images of 100 objects into Rekognition API to collect object labels, and analyzed the collected labels semantically to identify the labels that can be considered as ground truth. For example, a Coca Cola object can be recognized as a beverage, a bottle, a drink, a coke, a soda, or a glass. We selected 4 objects from each object category based on the number of images that can be correctly identified by Rekognition API. If a selected object was similar to another object in the same category, the object with more correctly identified images was utilized. In total, we tested the performance of Amazon Rekognition with $150,000$ images. There were 6,000 ($24~objects~\times~5~backgrounds~\times~5~devices~\times~5~orientations$ $~\times~2~color/grayscale$  ) challenge-free images and 144,000 ($24~objects~\times~5~backgrounds~\times~5~devices~\times~5~orientations$ $~\times~2~color/grayscale~\times~8~ challenge~types~\times~3~challenge$ $~levels$) images with controlled challenging conditions. We limited the number of tested objects to minimize the total cost of experimentation.




 %The images of the 24 objects of all challenge types and levels are then passed as input to Rekognition, and the output is analyzed by checking for the appearance of ground truth labels and their confidence levels compared to those of other labels.


   
 
 %but with more images that have at least one ground truth label, the object is neglected and the selection process continues with an object that has the next higher number of images with ground truth labels. 
 

\vspace{1mm}
\noindent{\bf Performance Metrics:} Top-5 accuracy metric was employed to measure the recognition performance. Outputs of both APIs were sorted based on their confidence levels and the highest 5 labels were selected for top-5 accuracy calculation. If multiple labels shared the same confidence level as the $5^{th}$ label, they were also included. If a ground truth label was among the top list, it was considered as a correct prediction. After repeating this procedure for all the images, we calculated the ratio between the number of correct predictions and the total number of object images to obtain the overall top-5 accuracy. In addition to the overall recognition performance in terms of top-5 accuracy, we also provided confusion matrices for different challenge levels to analyze misclassifications. Each row of the matrix corresponds to instances of actual categories and each column of the matrix corresponds to instances of predicted categories. An ideal classifier would have a confusion matrix with a highlighted main diagonal. Each element in the confusion matrix is colored based on the classification accuracy according to the legend next to each figure. Since both recognition APIs do not provide a comprehensive list of possible labels, the labels that did not belong to any categories were excluded.

\begin{comment}
Specifically, a confusion matrix shows the mismatch between the actual and predicted categories. To obtain a confusion matrix, we compared the predicted label with the highest confidence to ground truth labels. In case of multiple labels with the same confidence, all of them were considered. If the label(s) with the highest confidence level matched ground truth labels of its actual category, we added one to corresponding diagonal entry. If there was no match, the predicted label was compared to the ground truth labels of other categories. When the label appeared in multiple categories, the score was distributed evenly among all categories with a match. 
\end{comment}




%This metric does not penalize the performance of the application for having a low confidence level as long as the corresponding ground truth label gets detected within the top 5 labels.

 
\subsection{Recognition Performance}

% 1. Performance vs. challenge levels by challenge types (color/grayscale separate plots)
% 2. Performance vs. challenge levels by object orientations -> one plot per challenge (color images only)
% In this section, we analyze the recognition performance with respect to different challenge types and levels. Moreover, we discuss the object categorical misclassifications as challenge level increases. Recognition performance corresponding to each challenge type and level is reported in Fig. \ref{fig:challenges_accuracy}. The object categorical misclassification is reported with confusion matrices in Fig. \ref{fig:confusion_mat_common}. In both figures, the first row corresponds to AMZN and the second to MSFT.

In this section, we analyze the performance of both recognition platforms under challenging conditions. We report the recognition performance using color and grayscale images of top and common objects in Fig. \ref{fig:challenges_accuracy}. Moreover, we discuss the misclassification between object categories under varying challenge levels with confusion matrices in Fig. \ref{fig:confusion_mat_common}. Lastly, we report the overall recognition performance of both platforms in Table \ref{tab_overall_results}.



\noindent{\bf Color versus Grayscale:} To understand the contribution of color in terms of recognition performance, Fig. \ref{fig:challenges_accuracy}(a) can be compared with Fig. \ref{fig:challenges_accuracy}(b) for Amazon, and Fig. \ref{fig:challenges_accuracy}(d) with Fig. \ref{fig:challenges_accuracy}(e) for Microsoft. Based on the results in Fig. \ref{fig:challenges_accuracy}, we observe that both recognition platforms utilize color information. However, color information affects overall recognition performance more significantly for Microsoft compared to Amazon.

% When color and grayscale performances are compared for challenge-free images, it is observed that recognition accuracy is slightly higher with color information for AMZN, and. This slight performance enhancement shows that color information is used by Amazon Rekognition but the contribution of color is not as critical as structural information coming from grayscale images. 


\vspace{1mm}
\noindent{\bf Challenging Conditions:} For both platforms, \emph{resizing} affects the performance the least for the 4 challenge levels present. \emph{Blur}, \emph{salt \& pepper} noise, and \emph{dirty lens 1} challenging conditions are the most effective in degrading the performance, leading to less than 1\% top-5 accuracy for Amazon and 0.1\% for Microsoft. In general, the challenges that remove structural components in an image degrade the application performance significantly. \emph{Blur} filters out high-frequency components and \emph{salt \& pepper} noise replaces random pixel values that corrupt structural components, which are critical for recognition task. Even though \emph{resizing} also filters out high-frequency components, the level of smoothing is not as remarkable as \emph{blur} and most structural components are preserved. \emph{Dirty lens 1} challenge overlays a dirty lens pattern with different weights corresponding to challenge levels, which effectively block edge and texture in an image. We also report the recognition performance using color images of 10 common objects in Fig.~\ref{fig:challenges_accuracy}(c) and Fig.~\ref{fig:challenges_accuracy}(f). Similar to top object performance, Amazon significantly outperforms Microsoft in all categories.

% For both color and grayscale images, \emph{resizing} and \emph{underexposure} categories result in the least degradation in performance, less than 8\% decrease between challenge-free and challenge level 3 performance. Challenging conditions including \emph{overexposure} and \emph{contrast} lead to 20\% decrease in performance followed by the \emph{dirty lens} challenges. \emp{Dirty lens} type 2 degrades the performance by about 25\%  whereas type 1 leads to 37\% decrease in accuracy. The most significant degradation in recognition accuracy is caused by \emph{salt and pepper noise} and \emph{blur} categories, more than 40\%.  
  
% In general, the challenges that remove or corrupt structural components degrade recognition performance significantly. \emph{Salt and pepper noise} removes random pixel values that corrupt high-frequency components and \emph{blur} filters out high-frequency components that are critical for recognizing shapes. Therefore, these two challenge categories lead to the most significant performance degradation as expected. Even though \emph{resizing} also smooths out high-frequency components, the level of smoothing is less significant compared to \emph{blur} challenge. In \emph{dirty lens 1}  category, a single dirt pattern is overlaid on original images and an increase in overlay weight corresponds to challenge level. Therefore, recognition performance linearly decreases as challenge level increases. However, in \emph{dirty lens 2}  category, a distinct dirt pattern is overlaid for each level, which leads to a piece-wise linear behavior since dirt patterns at different locations affect recognition differently. Challenging conditions including \emph{underexposure} and \emph{overexposure} alter pixel values but preserve monotonic relationships, which include sufficient structural information at lower challenge levels. 



\begin{figure}[htbp!]
\vspace{-2mm}
\begin{minipage}[b]{0.30\linewidth}
  \centering
\includegraphics[width=\textwidth]{./Figs/cTypesLevels/AWS_selObj23_color.pdf}\vspace{-1mm}
  \centerline{\footnotesize{(a) AMZN: Top obj-C}}\vspace{1mm}%\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.30\linewidth}
  \centering
\includegraphics[width=\textwidth]{./Figs/cTypesLevels/AWS_selObj23_grayscale.pdf}\vspace{-1mm}
  \centerline{\footnotesize{(b) AMZN: Top obj-G}}\vspace{1mm}%\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.30\linewidth}
  \centering
\includegraphics[width=\linewidth]{./Figs/cTypesLevels/AWS_comObj_color.pdf}\vspace{-1mm}
  \centerline{\footnotesize{(c) AMZN: Common obj-C}}\vspace{1mm}%\medskip
\end{minipage}
\begin{minipage}[b]{0.30\linewidth}
  \centering
\includegraphics[width=\linewidth]{./Figs/cTypesLevels/Azure_selObj23_color.pdf}\vspace{-1mm}
  \centerline{\footnotesize{(d) MSFT: Top obj-C}}\vspace{2mm}%\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.30\linewidth}
  \centering
\includegraphics[width=\linewidth]{./Figs/cTypesLevels/Azure_selObj23_grayscale.pdf}\vspace{-1mm}
  \centerline{\footnotesize{(e) MSFT: Top obj-G}}\vspace{2mm}%\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.30\linewidth}
  \centering
\includegraphics[width=\linewidth]{./Figs/cTypesLevels/Azure_comObj_color.pdf}\vspace{-1mm}
  \centerline{\footnotesize{(f) MSFT: Common obj-C} }\vspace{2mm}%\medskip
\end{minipage}
\centering
\includegraphics[width=\linewidth, trim= 10mm 5mm 10mm 0mm]{./Figs/Legend_two_rows.pdf}\vspace{1mm}
\caption{Accuracy of recognition platforms versus challenging conditions for color (C) and grayscale (G) images.}\vspace{-2mm}
\label{fig:challenges_accuracy}
\end{figure}


\vspace{1mm}
\noindent{\bf Misclassification:} We analyze the object categorical misclassifications at different challenge levels with confusion matrices as shown in Fig. \ref{fig:confusion_mat_common}, where the first row corresponds to Amazon Rekognition and the second row corresponds to Microsoft Azure. We observe that the main diagonals of Amazon Rekognition are more predominant than the diagonals of Microsoft Azure at every challenge level. As the challenge level increases, highlights in the main diagonals significantly diminish, which shows the vulnerabilities of the recognition platforms under challenging conditions. 
% In addition to changes in recognition performance with respect to challenge types and levels, we also analyze the misclassification between object categories under varying challenge levels. To analyze misclassificaiton, we provide a confusion matrix for each challenge level as shown in Fig. \ref{fig:confusion_mat_common}. Fig.~\ref{fig:confusion_mat_common}(a) includes all challenge-free color and grayscale images whereas Fig.~\ref{fig:confusion_mat_common}(b)-(d) include color and grayscale images of levels $1$, $2$ and $3$ from all challenge types. While the main diagonal is predominant in all matrices, the degree of predominance decreases and some non-diagonal elements start to become more visible as the challenge level increases.    
% 2 rows, 3 figures per row

\begin{figure}[h]
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[width=\textwidth, trim = 5mm 5mm 5mm 2mm]{./Figs/AWS_result/Confusion_Matrix/lev0_top1_cf.pdf}
  
  \centerline{\footnotesize{(a) AMZN: Lev\_0 }}\vspace{0mm}%\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[width=\textwidth, trim = 5mm 5mm 5mm 2mm]{./Figs/AWS_result/Confusion_Matrix/lev1_top1_cf.pdf}
  
  \centerline{\footnotesize{(b) AMZN: Lev\_1}}\vspace{0mm}%\medskip
  \end{minipage}
\hfill
\begin{minipage}[b]{0.23\linewidth}
  \centering
  \includegraphics[width=\linewidth, trim = 5mm 5mm 5mm 2mm]{./Figs/AWS_result/Confusion_Matrix/lev3_top1_cf.pdf}
  \vspace{0.01 cm}
  \centerline{\footnotesize{(c) AMZN: Lev\_3}}\vspace{0mm}%\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[width=\linewidth, trim = 5mm 5mm 5mm 2mm]{./Figs/AWS_result/Confusion_Matrix/lev5_top1_cf.pdf}
  \vspace{0.01 cm}
  \centerline{\footnotesize{(d) AMZN: Lev\_5}}\vspace{0mm}%\medskip
\end{minipage}
\hfill
\vspace{1mm}
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[width=\textwidth, trim = 5mm 5mm 5mm 5mm]{./Figs/Azure_result/Confusion_Matrix/lev0_top1_cf.pdf}
  
  \centerline{\footnotesize{(e) MSFT: Lev\_0}}\vspace{0mm}%\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[width=\textwidth, trim = 5mm 5mm 5mm 5mm]{./Figs/Azure_result/Confusion_Matrix/lev1_top1_cf.pdf}
  
  \centerline{\footnotesize{(f) MSFT: Lev\_1}}\vspace{0mm}%\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[width=\linewidth, trim = 5mm 5mm 5mm 5mm]{./Figs/Azure_result/Confusion_Matrix/lev3_top1_cf.pdf}
  \vspace{0.01 cm}
  \centerline{\footnotesize{(g) MSFT: Lev\_3}}\vspace{0mm}%\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[width=\linewidth, trim = 5mm 5mm 5mm 5mm]{./Figs/Azure_result/Confusion_Matrix/lev5_top1_cf.pdf}
  \vspace{0.01 cm}
  \centerline{\footnotesize{(h) MSFT: Lev\_5}}\vspace{0mm}%\medskip
  \end{minipage}
\centering
\vspace{-1mm}\includegraphics[width=\linewidth, clip, trim=10mm 2mm 25mm 0mm ]{./Figs/Legend_objCat.pdf}
\caption{Confusion matrix for object category classification at different challenge levels.}\vspace{-5mm}
\label{fig:confusion_mat_common}
\end{figure}


\vspace{1mm}
\noindent{\bf Overall Performance:} We report the overall recognition performance of Amazon Rekognition and Microsoft Azure in Table \ref{tab_overall_results}. Test sets include challenge images as well as original images and performance is reported in terms of top-5 accuracy. For Amazon Rekognition, we report the results for 10 common objects and 23 top objects as described in Section~\ref{subsec:challenge_setup}. For Microsoft Azure, we also report the results for the entire \texttt{CURE-OR} dataset. Amazon Rekognition shows significantly higher performance compared to Microsoft Azure for the top and common objects in both color and grayscale. Both recognition platforms show slightly better accuracy for the 10 common objects than the 23 top objects because the objects that can be recognized by both platform lead to a slightly higher average accuracy compared to remaining objects from top objects. When all objects are considered, Microsoft Azure's performance degrades even more, getting closer to 1\% top-5 accuracy because majority of the remaining 77 objects are not accurately recognized even when they are challenge-free. 

\begin{table}[b]\vspace{-3mm}
\footnotesize 
\centering
\caption{Overall recognition performances.}
\label{tab_overall_results}
\begin{tabular}{c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{} & \multicolumn{3}{c|}{Color} & \multicolumn{3}{c}{Grayscale} \\ \cline{2-7} 
 & Top & Common & All & Top& Common& All \\ \hline
\begin{tabular}[c]{@{}c@{}}AMZN\end{tabular} & 25.78 & 26.03 & - & 22.78 & 23.6 & - \\ \hline
\begin{tabular}[c]{@{}c@{}}MSFT\end{tabular} & 5.66 & 7.62 & 1.83 & 3.58 & 5.17 & 1.01 \\ \hline
\end{tabular}
\end{table}
% \vspace{-2mm}










==> Preprint for arXiv/main_2.tex <==
\subsection{Experimental Setup}

\noindent{\bf Image Quality Algorithms, Databases and Distortions:} We utilize three different types of full-reference image quality assessment algorithms including PSNR as a fidelity measure, SSIM \cite{Wang2004} as a structural similarity measure, and UNIQUE \cite{Temel_UNIQUE} as a data-driven quality measure based on color and structure. We validate the subjective quality estimation performance over LIVE \cite{live}, MULTI \cite{multi}, and TID13 \cite{tid} databases, which include $4,432$ images and $30$ distortion types. Distortion types in test databases can be grouped into 7 main categories as \emph{lossy compression}, \emph{image noise}, \emph{communication error}, \emph{image blur}, \emph{color artifacts}, \emph{global distortions} (intensity shift/contrast change), and \emph{local distortions}. 



\begin{comment}
\begin{table}[htbp!]
\small
\centering
\caption{Recognition accuracy and subjective quality estimation performance of image quality assessment algorithms in terms of Spearman correlation.}
\label{tab_perf}
\begin{tabular}{c|ccc} \hline

 & \textbf{PSNR}& \textbf{SSIM}  & \textbf{UNIQUE}   \\ \hline \hline
\multicolumn{1}{c|}{\textbf{Challenge Type}}  & \multicolumn{3}{c}{\textbf{Recognition Accuracy Estimation}} \\ \hline \hline
\bf Resize   &\bf 0.532  &0.150  &0.320   \\
\bf Underexposure   &0.216  &\bf 0.256  &0.193   \\ 
\bf Overexposure   &0.526  &\bf 0.550  &0.538   \\ 
\bf Blur   &0.792  &0.751  &\bf 0.928   \\ 
\bf Contrast   &\bf 0.785  &0.673  & 0.738  \\ 
\bf Dirty lens 1   &\bf 0.909  &0.823  &0.811   \\ 
\bf Dirty lens 2   &\bf 0.820  &0.595  &0.613   \\ 
\bf Salt \& Pepper   &\bf 0.757  &0.685  &0.693    \\ \hline
\bf Weighted Average   &\bf  0.963 &0.724  &0.632    \\ \hline  \hline
\textbf{Image Quality Databases} & \multicolumn{3}{c}{\textbf{Subjective Quality Estimation}}                                   \\ \hline \hline
\bf Compression   &0.871  &\bf 0.938    &0.934  \\ 
\bf Noise   &0.774  & 0.862  &\bf 0.875  \\ 
\bf Communication   &0.863  &0.931   &\bf 0.933  \\ 
\bf Blur   &0.803  & 0.905 &\bf 0.909  \\ 
\bf Color   &0.815  &0.235    & \bf 0.909 \\ 
\bf Global   &0.340  &\bf 0.499    & 0.356 \\ 
\bf Local   &0.543  &0.288   &\bf  0.645 \\ \hline
\bf Weighted Average   &0.745  &0.800   & \bf 0.881 \\ \hline

\end{tabular}
\end{table}

\end{comment}











\vspace{1mm}
\noindent{\bf Estimation Performance Calculation:} In this study, we estimate the recognition accuracy with respect to changes in photometric conditions. The top-5 accuracy results from Amazon Rekognition and Microsoft Azure were averaged for this section. At first, we identify the challenge-free images as references, which lead to the highest recognition accuracy. Then, we investigate the relationship between image quality and recognition accuracy. Specifically, first, we group images that are captured with a particular  device (5) in front of a specific backdrop (3) under a specific challenge level (6), which leads to 90 image groups for each challenge type. Each image group includes images of 10 common objects described in Section \ref{subsec:challenge_setup} for all orientations. Second, we calculate average recognition performance and image quality scores for each image group. Overall, for each challenge category, we obtain 90 image quality and recognition accuracy scores, which correspond to the average of image groups. Real-world living room and office backgrounds are excluded because performance in these backgrounds are significantly different from other backgrounds, which cannot be captured with quality estimators that require pixel-to-pixel correspondence. Third, we calculate the Spearman correlation between objective quality and recognition accuracy scores to obtain recognition accuracy estimation performance. Moreover, we calculate the Spearman correlation between objective and subjective scores in image quality databases (LIVE, MULTI, and TID13) to obtain subjective quality assessment performance of image quality assessment (IQA) algorithms. 



\begin{table}[htbp!]
\small
\centering
\caption{Spearman correlation between average recognition accuracies and objective quality scores in the \texttt{CURE-OR} dataset.}
\label{tab_perf_recognition}
\begin{tabular}{c|ccc} \hline \hline
\textbf{Challenge Type} & \textbf{PSNR}& \textbf{SSIM}  & \textbf{UNIQUE}   \\ \hline \hline 
\bf Resize   & \bf0.755 & 0.382 & 0.312    \\
\bf Underexposure    & 0.722 & \bf0.807 & 0.407   \\ 
\bf Overexposure   & \bf0.642 & 0.432 & 0.576 \\ 
\bf Blur   & 0.782 & 0.749 & \bf0.876 \\ 
\bf Contrast   & \bf0.813 & 0.644 & 0.767 \\ 
\bf Dirty lens 1  & \bf0.915 & 0.872 & 0.841  \\ 
\bf Dirty lens 2  & \bf0.911 & 0.667 & 0.643  \\ 
\bf Salt \& Pepper   & \bf0.792 & 0.791 & 0.780 \\ \hline
%\bf Weighted Average   &\bf  0.963 &0.724  &0.632    \\ \hline  \hline
\end{tabular}
\end{table}
 \vspace{-2mm}

\subsection{Recognition Accuracy and Subjective Quality Estimation}
We report the recognition accuracy estimation in Table~\ref{tab_perf_recognition}  and subjective quality estimation in Table~\ref{tab_perf_quality}. In terms of challenge categories, PSNR is leading in majority of the categories whereas SSIM is leading in \emph{underexposure} category and UNIQUE in \emph{blur} category. Overall,  fidelity-based PSNR has the highest correlation, SSIM is the second measure, and UNIQUE is the third measure. Moreover, the relationship between the average recognition accuracy of both APIs on common objects and the quality scores can be observed from the scatter plots in Fig.~\ref{fig:scatter}. Scatter point distribution has a linear characteristic in PSNR whereas scatter points are more spread out for other quality measures. Even though SSIM and UNIQUE do not show a linear behavior, we can observe that scatter points corresponding to different challenge levels form distinct clusters. Therefore, UNIQUE and SSIM scores combined with top-5 accuracy scores can be informative in terms of identifying challenge level of the scenes.




\begin{comment}

\begin{figure}[!htbp]
\begin{minipage}[b]{0.32\linewidth}
  \centering
\includegraphics[width=\textwidth]{./Figs/Confusion_Matrix/lev0_top1_cf.pdf}
  \vspace{0.01cm}
  \centerline{\footnotesize{(a) Challenge Free}}%\medskip
\end{minipage}
\begin{minipage}[b]{0.32\linewidth}
  \centering
\includegraphics[width=\textwidth]{./Figs/Confusion_Matrix/lev1_top1_cf.pdf}
  \vspace{0.01cm}
  \centerline{\footnotesize{(b) Level 1}}%\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.32\linewidth}
  \centering
\includegraphics[width=\textwidth]{./Figs/Confusion_Matrix/lev2_top1_cf.pdf}
  \vspace{0.01 cm}
  \centerline{\footnotesize{(c) Level 2}}%\medskip
\end{minipage}
\centering
% \includegraphics[width=\linewidth]{./Figs/Legend_w_average.pdf}
  \vspace{-2.0mm}
\caption{Scatter plots of object recognition accuracy versus objective quality scores.}
\label{fig:s}
\end{figure}

\end{comment}

% trim: left bottom right top
\begin{figure}[htbp!]
\centering
    % \includegraphics[clip, trim=2cm 11cm 2cm 11cm, width=0.93\linewidth]{./Figs/IQAs_perf.pdf}
    %  \includegraphics[clip, trim=4cm 14cm 3cm 12.7cm, width=0.93\linewidth]{./Figs/IQAs_perf_legend.pdf}\vspace{-3mm}
    \includegraphics[clip, trim=2mm 2mm 1.5mm 1mm, width=0.32\linewidth]{./Figs/IQAs_perf_PSNR_allLev.pdf}
    \includegraphics[clip, trim=2mm 2mm 1.5mm 1mm, width=0.32\linewidth]{./Figs/IQAs_perf_SSIM_allLev.pdf}
    \includegraphics[clip, trim=2mm 2mm 1.5mm 1mm, width=0.32\linewidth]{./Figs/IQAs_perf_UNIQUE_allLev.pdf}
    \includegraphics[clip, trim=1.3cm 5mm 1.1cm 0mm, width=0.98\linewidth]{./Figs/IQAs_perf_legend_allLev.pdf}    
    \caption{Scatter plots of object recognition accuracy versus objective quality scores.}
    \label{fig:scatter}
    \vspace{-3mm}
\end{figure}



According to subjective quality estimation performances in the image quality databases reported in Table~\ref{tab_perf_quality},  UNIQUE leads to highest correlation in majority of the distortion types and SSIM leads in \emph{compression} and \emph{global} categories. SSIM and UNIQUE are specifically designed for estimating subjective quality of images whereas PSNR is used for calculating the fidelity of a general signal representation based on the ratio of maximum signal power and noise power. Therefore, UNIQUE and SSIM outperform PSNR in the application they are designed for whereas they underperform in estimating recognition accuracy. Even though objective quality assessment algorithms can estimate the recognition performance in certain scenarios, they are inherently limited because significant perceptual changes captured by quality assessment algorithms may not be critical for recognition algorithms.


\begin{table}[htbp!]
\small
\centering
\caption{Spearman correlation between subjective quality scores and objective quality scores in the IQA databases.}
\label{tab_perf_quality}
\begin{tabular}{c|ccc} \hline \hline
\textbf{Challenge Type} & \textbf{PSNR}& \textbf{SSIM}  & \textbf{UNIQUE}   \\ \hline \hline 
\bf Compression   &0.871  &\bf 0.938    &0.934  \\ 
\bf Noise   &0.774  & 0.862  &\bf 0.875  \\ 
\bf Communication   &0.863  &0.931   &\bf 0.933  \\ 
\bf Blur   &0.803  & 0.905 &\bf 0.909  \\ 
\bf Color   &0.815  &0.235    & \bf 0.909 \\ 
\bf Global   &0.340  &\bf 0.499    & 0.356 \\ 
\bf Local   &0.543  &0.288   &\bf  0.645 \\ \hline
%bf Weighted Average   &0.745  &0.800   & \bf 0.881 \\ \hline \hline
\end{tabular}
\vspace{-3mm}
\end{table}

\begin{comment}

\begin{table}[htbp!]
\footnotesize
\centering
\caption{Recognition accuracy and subjective quality estimation performance of image quality assessment algorithms in terms of Spearman correlation.}
\label{my-label}
\begin{tabular}{c|cccc} \hline

 & \textbf{PSNR}& \textbf{SSIM} & \textbf{PerSIM}  & \textbf{UNIQUE}   \\ \hline
\multicolumn{1}{c|}{\textbf{Challenge Type}}  & \multicolumn{4}{c}{\textbf{Recognition Accuracy Estimation}} \\ \hline

\bf Underexposure   &  &  &  &  \\ 
\bf Overexposure   &  &  &  &  \\ 
\bf Blur   &  &  &  &  \\ 
\bf Contrast   &  &  &  &  \\ 
\bf Dirty lens 1   &  &  &  &  \\ 
\bf Dirty lens 2   &  &  &  &  \\ 
\bf Salt \& Pepper   &  &  &  &  \\ \hline
\bf Average   &  &  &  &  \\ \hline

\textbf{Image Quality Databases} & \multicolumn{4}{c}{\textbf{Subjective Quality Estimation}}                                   \\ \hline
\bf Compression   &0.871  &0.938  &0.935  &0.934  \\ 
\bf Noise   &0.774  & 0.862 & 0.917 &0.875  \\ 
\bf Communication   &0.863  &0.931  &0.918  &0.933  \\ 
\bf Blur   &0.803  & 0.905 & 0.892 &0.909  \\ 
\bf Color   &0.815  &0.235  &0.762  & 0.909 \\ 
\bf Global   &0.340  &0.499  &0.409  & 0.356 \\ 
\bf Local   &0.543  &0.288  &0.471  & 0.645 \\ \hline
\bf Average   &0.745  &0.800  &0.871  & 0.881 \\ \hline



%\bf LIVE  &0.909  &0.950  &0.950  &0.952  \\ \hline
%\bf MULTI  &0.677  &0.860  &0.818  &0.867  \\ \hline
%\bf TID13  &0.701  &0.742  &0.854  &0.860  \\ \hline



\end{tabular}
\end{table}

\end{comment}

==> Preprint for arXiv/related_work.tex <==
\input{tab_datasets}
There are numerous datasets in the literature that can be used to benchmark the performance of object recognition algorithms. We can classify these datasets into two categories as \emph{controlled} datasets and \emph{uncontrolled} datasets. In \emph{uncontrolled} 
datasets \cite{Li2004,Opelt2005, Everingham2005,Russell2008,Torralba2008,Krizhevsky09,Deng2009,Saenko2010,Lin2014}, images are commonly acquired through search engines or photo sharing platforms. \emph{Uncontrolled} datasets are advantageous because it is easier to obtain large-scale datasets that include varying environmental conditions. The variety of images in these \emph{uncontrolled} datasets enables a large-scale performance assessment of algorithms. However, because of their \emph{uncontrolled} nature, it is not possible to understand the specific factors that affect recognition performance in these datasets.


\begin{figure}[b]
%  \vspace{-2mm}
    \centering \includegraphics[width=0.61\linewidth, trim= 35mm 48mm 35mm 40mm]{./Figs/datasets_v6.pdf} 
    \caption{An overview of object datasets in terms of dataset size and number of annotated controlled conditions.} %\vspace{-1mm}
    \label{fig:scatter_cure}
\end{figure}


In \emph{controlled} datasets \cite{Nene1996,Funt1998,Koubaroulis2002,Ferrari2004,LeCun2004,Geusebroek2005,Lai2011,Singh2014,Borji2016}, images are captured in a restricted setup under varying conditions. COIL-100 \cite{Nene1996}, SFU \cite{Funt1998}, SOIL-47 \cite{Koubaroulis2002}, and ETHZ Toy \cite{Ferrari2004} datasets contain up to thousands of images, which are limited compared to \emph{uncontrolled} recognition datasets. On the other hand, ALOI \cite{Geusebroek2005}, NORB \cite{LeCun2004}, RGB-D \cite{Lai2011}, and BigBIRD \cite{Singh2014} datasets are large-scale but their controlled conditions are limited to relative camera location, rotation, or lighting. Among all aforementioned \emph{controlled} datasets, iLab-20M \cite{Borji2016} is the largest dataset with a variety of acquisition conditions including relative camera location, focus level, scale, and background. In iLab-20M, one type of camera is used in the data acquisition, which makes the study overlook the domain differences that can be caused by acquisition device type as shown in \cite{Saenko2010}. Moreover, iLab-20M  is mainly used to test the invariance of learning-based approaches rather than analyzing factors that can affect the recognition performance, which is not possible to investigate until the data is publicly available. We summarize the main characteristics of existing datasets as well as introduced dataset \texttt{CURE-OR} in Table~\ref{tab_datasets} and compare these datasets in terms of number of images and annotated controlled conditions in Fig. \ref{fig:scatter_cure}. Because of the significant difference between the number of images in different datasets, we visualize data points in log scale. Ideally, a test dataset should be located on the top right corner so that it will be large-scale in terms of the number of images and annotated challenge types and levels. iLab-20M  and \texttt{CURE-OR}  are closest to top right with respect to compared datasets.









%such as COIL-100 \cite{Nene1996}, SFU \cite{Funt1998}, SOIL-47 \cite{Koubaroulis2002}, ETHZ Toys \cite{Ferrari2004}, NORB \cite{LeCun2004}, ALOI \cite{Geusebroek2005}, BigBIRD \cite{Singh2014}, and iLab-20M \cite{Borji2016},












%such as Caltech101 \cite{Li2004}, PASCAL \cite{Everingham2005}, CIFAR \cite{Krizhevsky09} and ImageNet \cite{Deng2009}, images were acquired through search engines or photo sharing platforms.

 






%controlled conditions including but not limited to background, point of view, or lighting. 









%\texttt{CURE-OR} is a large-scale object recognition dataset introduced in this study. In Fig. \ref{fig:object_datasets}, we report the number of images along with number of annotated challenge types of existing datasets along with \texttt{CURE-OR} dataset. Because of the significant difference between number of images in different datasets, we visualize data points in log scale. Ideally, a test dataset should be located on the top right corner so that it will be large scale and include numerous challenging conditions with metadata. 
%iLab-20M \cite{Borji2016} and \texttt{CURE-OR}  are closest to top right compared to all other datasets. 



==> Preprint for arXiv/tab_datasets.tex <==
\begin{table*}[]
\footnotesize

\centering
\caption{Main characteristics of publicly available object datasets and \texttt{CURE-OR}.}

\label{tab_datasets}
\begin{tabular}{>{\centering\arraybackslash}p{1.4cm}|>{\centering\arraybackslash}p{0.7cm}>{\centering\arraybackslash}p{1.1cm}>{\centering\arraybackslash}p{1.05cm}>{\centering\arraybackslash}p{1.4cm}>{\centering\arraybackslash}p{1.1cm}>{\centering\arraybackslash}p{1.0cm}>{\centering\arraybackslash}p{1.1cm}>{\centering\arraybackslash}p{1.4cm}>{\centering\arraybackslash}p{1.2cm}>{\centering\arraybackslash}p{1.3cm}}
\hline

 
 &   \textbf{\begin{tabular}[c]{@{}c@{}}Release \\ year\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number\\ of\\ images\end{tabular}} & \textbf{Resolution} &  \textbf{\begin{tabular}[c]{@{}c@{}}Object \\ classes \end{tabular}} &\textbf{\begin{tabular}[c]{@{}c@{}}Number of\\ images per\\ class\end{tabular}}&\textbf{\begin{tabular}[c]{@{}c@{}}Number of\\different\\ objects per\\ class\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number of \\ images per \\ same object\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Controlled \\ condition\\ (level)\end{tabular}} & \textbf{Background} & \textbf{Acquisition}  \\ \hline
 

 
\textbf{\href{http://www.cs.columbia.edu/CAVE/software/softlib/coil-100.php}{COIL100}}  & 1996   & 7,200 &128x128  &household  &\begin{tabular}[c]{@{}c@{}}all\\images \end{tabular}  & 100 &72  & \begin{tabular}[c]{@{}c@{}}angle (72)\\ \end{tabular}  &black  & \begin{tabular}[c]{@{}c@{}}CCD cam. \end{tabular}\\ \hline








\textbf{\href{http://www.cs.sfu.ca/~colour/image\_db/index.html}{SFU}}   & 1998   &\begin{tabular}[c]{@{}c@{}}all\\images \end{tabular} &637x468  &household &110 &11  &10  &\begin{tabular}[c]{@{}c@{}}lighting (5)\\ position (2) \end{tabular}  &black  & \begin{tabular}[c]{@{}c@{}}CCD cam.  \end{tabular} \\ \hline






\textbf{\href{http://www.cs.sfu.ca/~colour/image\_db/index.html}{SOIL-47}}   &2002   &\begin{tabular}[c]{@{}c@{}}all\\images \end{tabular}  & \begin{tabular}[c]{@{}c@{}}288x360 \\ and\\ 576x720\end{tabular}  & household &1,974 & 47 & 42 &\begin{tabular}[c]{@{}c@{}}angle (21)\\ lighting (2)\end{tabular}  & black &\begin{tabular}[c]{@{}c@{}}CCD cam. \end{tabular} \\ \hline








\textbf{\href{http://calvin.inf.ed.ac.uk/datasets/ethz-toys/}{ETHZ Toys}}  &2004  &63&720x576 &household  &\begin{tabular}[c]{@{}c@{}}all\\images \end{tabular} &9 &1-8 &angle (1-8) & \begin{tabular}[c]{@{}c@{}}black (model)\\ generic (test)\end{tabular}&- \\ \hline



\textbf{\href{http://www.cs.nyu.edu/~ylclab/data/norb-v1.0/}{NORB}} & 2004  &194,400  &640x480  & \begin{tabular}[c]{@{}c@{}}toys:  \\airp., trucks \\cars, human fig. \\four-leg. anim. \end{tabular}  &38,880  &10  & 3,888 &  \begin{tabular}[c]{@{}c@{}}angle (9)\\ azimuth (18)\\ lighting (6)\end{tabular} & \begin{tabular}[c]{@{}c@{}}white\\ textured\end{tabular} &\begin{tabular}[c]{@{}c@{}}2 CCD \\ cameras\end{tabular}  \\ \hline


\textbf{\href{http://www.vision.caltech.edu/Image\_Datasets/Caltech101/}{CalTech 101}}   &2004   &9,145  &300x200  &101 generic  &40-800& - & - & NA  &generic  & \begin{tabular}[c]{@{}c@{}}Online\\ search\end{tabular}  \\ \hline








\textbf{\href{http://host.robots.ox.ac.uk/pascal/VOC/voc2005/index.html}{PASCAL VOC}}  &2005   &2,232  & \begin{tabular}[c]{@{}c@{}}110x75 \\ to\\ 1,280x960\end{tabular} & \begin{tabular}[c]{@{}c@{}}motorcycles\\ bicycles\\ people\\ cars\end{tabular}  &168-547 &-  &-  & NA & generic & \begin{tabular}[c]{@{}c@{}}Online\\ search \\ETHZ\\UIUC  \end{tabular}  \\ \hline



\textbf{\href{http://www.emt.tugraz.at/~pinz/data/GRAZ\_02/}{GRAZ-02}}  & 2005 &1,476& \begin{tabular}[c]{@{}c@{}}480x640 \\ 640x480\end{tabular}&\begin{tabular}[c]{@{}c@{}}person, bike\\cars, counter\end{tabular} &311-420 &- &- & NA &generic&-  \\ \hline



\textbf{\href{http://aloi.science.uva.nl/}{ALOI}}  &2005  &110,250&768x576 &small obj. &\begin{tabular}[c]{@{}c@{}}all\\images \end{tabular} &1,000&$>$100 & \begin{tabular}[c]{@{}c@{}} angle (72)\\ light. angle (24) \\ light. color (12)\end{tabular}&black &\begin{tabular}[c]{@{}c@{}}3 CCD \\ cameras\end{tabular}  \\ \hline

%\textbf{ETHZ} &- &2006  &255 &- &\begin{tabular}[c]{@{}c@{}}bottles, swans\\ mugs, giraffes,\\ apple logos\end{tabular} & &32-87 &- &-  &generic&\begin{tabular}[c]{@{}c@{}}Online search, \\ Flickr\end{tabular} &-  \\ \hline




\textbf{\href{http://labelme.csail.mit.edu/Release3.0/browserTools/php/dataset.php}{LabelME}} & 2008 &\begin{tabular}[c]{@{}c@{}}11,845 pic.\\ 18,524 fram.\end{tabular}&\begin{tabular}[c]{@{}c@{}}high\\resolution \end{tabular} &\begin{tabular}[c]{@{}c@{}}4,210\\ Wordnet\\categories \end{tabular}&\begin{tabular}[c]{@{}c@{}}up to\\27,719  \end{tabular} &- & - &NA&generic & \begin{tabular}[c]{@{}c@{}}Online\\ search\end{tabular} \\ \hline





\textbf{\href{http://groups.csail.mit.edu/vision/TinyImages/}{Tiny}}  &2008  &79,302,017&32x32 &\begin{tabular}[c]{@{}c@{}} 75,062  \\Wordnet \\nonabstract\\nouns \end{tabular} &\begin{tabular}[c]{@{}c@{}} up to \\3,000\end{tabular}&- &- &NA  &generic&\begin{tabular}[c]{@{}c@{}}Online\\search\end{tabular}  \\ \hline



\textbf{\href{https://www.cs.toronto.edu/~kriz/cifar.html}{CIFAR10 CIFAR100}}  &2009  &60,000&32x32 &\begin{tabular}[c]{@{}c@{}} 10 subclass of \\ vehic. and anim.,\\100 subclass of \\ 20 superclass  \end{tabular} & \begin{tabular}[c]{@{}c@{}} 6,000, \\600\end{tabular}  &- &- &NA&generic& \begin{tabular}[c]{@{}c@{}}Online\\search\end{tabular}  \\ \hline



\textbf{\href{http://image-net.org/}{ImageNet}}  &  2009 &3,200,000  & \begin{tabular}[c]{@{}c@{}}400x350 \\ (avg.) \end{tabular}  & \begin{tabular}[c]{@{}c@{}}5,247 \\Wordnet\\ synsets\end{tabular}  & \begin{tabular}[c]{@{}c@{}}600 \\ (avg.) \end{tabular}&-   & - &NA &generic  & \begin{tabular}[c]{@{}c@{}}Online\\ search\end{tabular}   \\ \hline


\textbf{\href{https://sites.google.com/site/bosstimuli/}{BOSS}} &  2010 &480  &2,000x2,000  &household  & \begin{tabular}[c]{@{}c@{}}all\\images \end{tabular}& 480 & 1 & NA &white  &-  \\ \hline




\textbf{\href{https://people.eecs.berkeley.edu/~jhoffman/domainadapt/\#datasets_code}{Office}}  &2010  &\begin{tabular}[c]{@{}c@{}}2,817 \\498\\795 \end{tabular}  & \begin{tabular}[c]{@{}c@{}}300x300 \\1,000x1,000 \\152x152 to \\752x752 \end{tabular}&\begin{tabular}[c]{@{}c@{}} 31 product  \\ categ.  \end{tabular}  &\begin{tabular}[c]{@{}c@{}}36-100 \\7-31  \\11-43 \end{tabular} &\begin{tabular}[c]{@{}c@{}}- \\4-6  \\4-6  \end{tabular}  &\begin{tabular}[c]{@{}c@{}}- \\ 1-9 \\1-14 \end{tabular}&\begin{tabular}[c]{@{}c@{}}NA\end{tabular} & \begin{tabular}[c]{@{}c@{}}studio light \\office env. \\office env.  \end{tabular}&\begin{tabular}[c]{@{}c@{}}Amazon.com\\DSLR cam.\\webcam \end{tabular}\\ \hline






\textbf{\href{http://rll.berkeley.edu/bigbird/}{BigBIRD}} & 2014  &150,000  &\begin{tabular}[c]{@{}c@{}}1,280x1,024 \\ 4,272x2,848\end{tabular}  &household &\begin{tabular}[c]{@{}c@{}}all\\images \end{tabular} &125  &1,200  & angle (120)  &white  & \begin{tabular}[c]{@{}c@{}}DSLR cam.\\ depth sensors\end{tabular}  \\ \hline








\textbf{\href{http://mscoco.org/}{MS-COCO}}  & 2014 &328,000& &\begin{tabular}[c]{@{}c@{}}91 classes \\incl. PACAL \\VOC 2011 \end{tabular} &\begin{tabular}[c]{@{}c@{}}3,600\\(avg)\\\end{tabular}  &- &-  &NA&generic &\begin{tabular}[c]{@{}c@{}}Online\\ search\end{tabular} \\ \hline



\textbf{iLab-20M}  &2016  &21,798,480&960x720 &\begin{tabular}[c]{@{}c@{}}toys \\ \end{tabular} &\begin{tabular}[c]{@{}c@{}}all\\images \end{tabular}  &704 &1,320  &\begin{tabular}[c]{@{}c@{}}angle (8) \\azimuth (11)\\focus (3)\\ lighting (5)\\backgr. ($>$14) \end{tabular}&\begin{tabular}[c]{@{}c@{}}textured \\backdr. (125), \\solid color\\backdr. (7) \end{tabular} &\begin{tabular}[c]{@{}c@{}}webcam (11) \\ \end{tabular} \\ \hline




\textbf{CURE-OR}   & 2018  &1,000,000 & \begin{tabular}[c]{@{}c@{}}648x968 \\756x1,008\\ 480x640\\460x816\\726x1,292 \end{tabular} & \begin{tabular}[c]{@{}c@{}} pers. belong.\\ office supply\\ household\\ toy \\sports/entert.\\health/pers.care \end{tabular}&\begin{tabular}[c]{@{}c@{}}100,000-\\270,000\end{tabular}  & 10-27  &10,000  & \begin{tabular}[c]{@{}c@{}} orientation (5)\\ backgr. (5)\\ challenge (79)\end{tabular} & \begin{tabular}[c]{@{}c@{}}white backdr.\\textured \\backdr (2),\\ living room \\ office\end{tabular} & \begin{tabular}[c]{@{}c@{}}DSLR cam. \\webcam\\phone(x3)\end{tabular} \\ \hline

%\textbf{} & &  && &&  & &  && & &\\ \hline

\end{tabular}
\end{table*}



